The first all-sky view of the Milky Way stellar halo with Gaia+2MASS RR Lyrae

We exploit the first \gaia data release to study the properties of the Galactic stellar halo as traced by RR Lyrae. We demonstrate that it is possible to select a pure sample of RR Lyrae using only photometric information available in the Gaia+2MASS catalogue. The final sample contains about 21600 RR Lyrae covering an unprecedented fraction ($\sim60\%$) of the volume of the Galactic inner halo ($\text{R}<28$ kpc). We study the morphology of the stellar halo by analysing the RR Lyrae distribution with parametric and non-parametric techniques. Taking advantage of the uniform all-sky coverage, we test halo models more sophisticated than usually considered in the literature, such as those with varying flattening, tilt and/or offset of the halo with respect to the Galactic disc. A consistent picture emerges: the inner halo is well reproduced by a smooth distribution of stars settled on triaxial ellipsoids. The minor axis is perpendicular to the Milky Ways disc, while the major axis is misaligned by $\sim20^{\circ}$ from the Galactic Y axis. The elongation along the major axis is mild ($\text{p}=1.27$), and the vertical flattening is shown to evolve from a squashed state with $\text{q}\approx0.57$ in the centre to a more spherical $\text{q}\approx0.75$ at the outer edge of our dataset. The density slope is well approximated by a single power-law with exponent $\alpha=-2.96$. Within the range probed, we see no significant evidence for a change of the radial density slope, out of the plane tilt or an offset of the halo with respect to the Galaxy's centre.

==> include/method_old.tex <==
\section{Model fitting}\ \label{sec:bay}
In this section we  present a and fit  the model describing the distribution of RRLs around the Galaxy.


\subsection{Clean sample} \label{sec:csample}

Figs.  \ref{fig:Rzdens} and \ref{fig:mb10} show  the  presence of  an highly  \vir{flattened} structure close to the Galactic plane. The properties of this structure are  clearly at  odds  with the distribution  of stars  at  high  Galactic latitude that are more  likely  a  \vir{genuine} tracer of the  halo population. 
The \vir{flattened} substructure  contains  a significant portion of  RRLs  in our sample (about the 35\%) and, 
if not  properly modelled, it can introduce severe biases  in the final results of our statistic analysis. Therefore, we decided to  obtain a  \vir{clean} sample of RRLs eliminating from  our original catalogue (Sec. \ref{sec:selection}) all the stars belonging to the substructure. 
There are different  selection cuts that we can  apply to
exclude these  stars, but  Fig. \ref{fig:mb10} shows that  the most  effective is  probably  a cut  on the angle $\theta$ (see definition in \ref{eq:fref2}). In particular  at $|\theta|=20^\circ$ (white-dashed line in Fig. \ref{fig:mb10}) is evident  a  transition  between a very flattened  component  and  a more  spheroidal  structure. 
We tried also a direct cut on  $\te{Z}_\te{g}$,  we found that to exclude most on the stars of the flattened substructure, we should remove all the objects with   $|\te{Z}_\te{g}|<4$ kpc. This cut reduces significantly the number of tracers in the very inner part of the halo, moreover we found that the final number of stars is smaller with respect to the cut at $|\theta|=20^\circ$.

In conclusion, we  obtained a  new sample of RRLs  keeping all the stars with $|\theta|>20^\circ$: this subsample contains  13713  objects  and covers about the  44\% of the  halo volume  within a sphere  with a radius of  28 kpc (see Tab. \ref{tab:tab_cut}).
In the following subsections we  present the method  used to fit  halo models to  these subsample of RRLs and  the  final results.
A more detailed analysis of the  cut substructure can be found in Sec. \ref{sec:struct}.




\subsection{Halo models} \label{sec:hmodel}
As already  done in Sec. \ref{sec:look}, we assumed that the  RRLs in the  halo  are settled  on ellipsoids  defined by the elliptical radius  $\te{r}_\te{e}$ (Eq. \ref{eq:ellrad}) so that the  density is function of  $\te{r}_\te{e}$ only.  The elliptical radius  depends  on the  assumption made  on the  shape of the ellipsoidal iso-density surfaces, in particular it depends on the  axial ratios q and p. Therefore, an  halo model  is defined  by a  functional form for the density law  and  
a \vir{geometrical} model for the ellipsoidal iso-density surfaces.

\subsubsection{Density profiles} \label{sec:densmod}
The distribution  of  stars in the halo  is usually  described with  a power-law density profile usually  showing   a change of  slope  between  the  inner  and  the outer parts. A very  flexible  way to  define  a  power-law profile is 
\begin{equation}
\rho(\te{r}_\te{e})\propto\left(  \frac{\te{r}_\te{e}}{\te{r}_\te{eb}}  \right)^{-\alpha_\te{inn}}  \left( 1+ \frac{\te{r}_\te{e}}{\te{r}_\te{eb}}  \right)^{-\alpha_\te{out}},
\label{eq:plgeneral}
\end{equation}
where $\alpha_\te{inn}$ and  $\alpha_\te{out}$ indicate the power-law  slopes and $\te{r}_\te{eb}$ is the scale length.
Two  extreme  cases can  be  obtained  from  Eq. \ref{eq:plgeneral}:
if we assume $\alpha_\te{out}=0$, Eq. \ref{eq:plgeneral} becomes  a simple power-law profile   $\rho \propto \te{r}_\te{e}^{-\alpha_\te{inn}}$ (SPL, hereafter); while, setting   $\alpha_\te{inn}=0$  we obtain a profile with a  inner core  with a scale length  $\te{r}_\te{eb}$ and  an  outer slope equal to $-\alpha_\te{out}$  (CPL, hereafter). All the other cases  represent intermediate  situations  where the density law is defined by   a profile with a double slope (DPL, hereafter), in particular it has an inner slope $-\alpha_\te{inn}$ for $\te{r}_\te{e}<<\te{r}_\te{eb}$  an outer slope $-(\alpha_\te{inn}+\alpha_\te{out})$ for $\te{r}_\te{e}>>\te{r}_\te{eb}$ and a transition region around $\te{r}_\te{e}\approx\te{r}_\te{eb}$. 

Instead  of  treating the change of slope as a smooth transition,  we can  assume  that  it happens  abruptly at certain  radius $\te{r}_\te{eb}$. In this case the density profile  is represented by the piece-wise  function  
\begin{equation}
\rho(\te{r}_\te{e})\propto
\begin{cases}
\te{r}_\te{e}^{-\alpha_\te{inn}} & \te{r}_\te{e}\leq\te{r}_\te{eb}  \\
\te{r}_\te{eb}^{\alpha_\te{out}-\alpha_\te{inn}} \te{r}_\te{e}^{-\alpha_\te{out}} & \te{r}_\te{e}\geq\te{r}_\te{eb}.
\end{cases}
\label{eq:bpl}
\end{equation}
We define the Eq. \ref{eq:bpl} a broken power-law (BPL, hereafter).

Eqs. \ref{eq:plgeneral} and \ref{eq:bpl}
 can describe density profiles with  one change  on slope at most.  In order to  test  a more  complicate behavior of the RRLs density law, we  consider also the Einasto density profile \citep{einastor} 
\begin{equation}
\rho(\te{r}_\te{e}) \propto \text{Exp} \left[ -d_\te{n} \left( \left( \frac{\te{r}_\te{e}}{\te{r}_\te{eb}} \right)^{\frac{1}{\te{n}}} -1 \right) \right],
\label{eq:einasto}
\end{equation}
where  $d_\te{n}=3\te{n} -0.3333 +0.0079/\te{n}$ for  $\te{n}\geq0.5$ \citep{einasto}.
The steepness of the Einasto  profile, $\alpha_\te{einasto}$, changes continuously as function of $\te{r}_\te{e}$ tuned by the  parameter $\te{n}$ 
\begin{equation}
\alpha_\te{einasto}=-\frac{d_\te{n}}{\te{n}} \left(   \frac{\te{r}_\te{e}}{\te{r}_\te{eb}} \right)^{\frac{1}{\te{n}}},
\label{eq:einastostep}
\end{equation}
so lower is n, larger is the variation of the slope in the analysed radial domain. For very small values  of $\te{n}$ ($\te{n}\leq2$), the profile shows almost an inner core up to the scale length $\te{r}_\te{eb}$ and then a rapid decrease. Contrarily for large values of $\te{n}$,  the variation of the slope is slow, so that with the right combination of  $\te{n}$ and $\te{r}_\te{eb}$  the Einasto profile can roughly  mimic a SPL profile in a certain  portion of the radial domain.    
\subsubsection{Iso-density ellipsoidal surfaces} \label{sec:ellsurf}
Once  the density model has been selected  the  final  likelihood  (Eq. \ref{eq:likel}) depends  only on the values  $\te{r}_\te{e}$  of  the stars in  our sample.
Therefore, the final result will depend   on the shape  of the iso-density ellipsoidal surfaces  through  the assumption on the  parameter  p and  q  (see Eq. \ref{eq:ellrad}). We define three different models:
\begin{itemize}
\item{Spherical,} we set $\te{p}=1$ and $\te{q}=1$ in  Eq. \ref{eq:ellrad},  so that  $\te{r}_\te{e}$ is  just  the  spherical  radius $\te{D}_\te{g}$ (see definition \ref{eq:fref2})   in the  Galactic  frame  of reference;
\item{Oblate,} in this model we set $\te{p}=1$ and  we consider the flattening along the Z-axis, q,  as free-parameter, we define this model Oblate because all the best-fit models have $\te{q}<1$ (see Tab. \ref{tab:fit});
\item{Prolate,} in this model we set $\te{q}=1$ and we  consider the flattening along the Y-axis, p, as free-parameter, we define this model Prolate because all the best-fit models have $\te{p}>1$ (see Tab. \ref{tab:fit});
\item{Triaxial:} in this model  both p and q  are considered free-parameters.
\end{itemize}

A number of works in literature found evidence of a change of  flattening  along the Z-axis, q,   as  a function  of the Galactic distance (e.g.  \citealt{das} and \citealt{xuehalo}), we found that this feature is also directly visible in the RRLs distribution (Fig. \ref{fig:mb10}).  Therefore, we  implemented the possibility to have a model with a non-constant q using the functional form
\begin{equation}
\te{q}(\te{r}_\te{e})=\te{q}_\infty - (\te{q}_\infty-\te{q}_0) \te{Exp}\left[ 1- \frac{\sqrt{\te{r}_\te{e}^2+\te{r}_\te{eq}^2}}{\te{r}_\te{eq}^2} \right],
\label{eq:qvar}
\end{equation}
where  q varies from  $\te{q}_0$ at the centre  to  the asymptotic  value  $\te{q}_\infty$ at large radii  and the variation is tuned by the  exponential scale length $\te{r}_\te{eq}$. There are no theoretical reasons to  use  Eq. \ref{eq:qvar} to trace the variation of  q, but  it has been  already used  by other authors  like  \cite{xuehalo} and \cite{das},  so we decided to use this function to have a direct comparison with their results. However, we note that both in  \cite{xuehalo} and \cite{das},  q is a function of the  spherical radius ($\te{D}_\te{g}$ as defined in \ref{eq:fref})  and not of the elliptical radius $\te{r}_\te{e}.$ We decided to maintain the dependence on $\te{r}_\te{e}$  given that this approach is self-consistent  with  our assumption that the RRLs are settled on  ellipsoidal surfaces.

Given the  unprecedented sky coverage of our sample, we tested, for the first time in  literature,  also  more complex models for the iso-density ellipsoidal surfaces. In particular  we took into account the possibility  to have a tilt of the  halo with respect  to the Galactic  plane  and an off-set  with   respect to the  Galactic centre.  
\begin{itemize}
\item{Tilted halo:} in this model  we assume that  the  symmetry  axis of the  ellipsoids  are not coincident  with the  X-Y-Z axes of the Galactic frame of reference; In practice, before to calculate the elliptical radii (Eq. \ref{eq:ellrad}), we transform the  Galactic coordinates (see definitions in \ref{eq:fref}) of each star applying a  rotation matrix $R(\eta,\beta,\gamma)$ following a  XYZ formalism so that  $\eta$ represents  the  rotation angle  around the  original X-axis,  $\beta$ the one  around the new  Y-axis and  finally $\gamma$ is the  rotation angle  around the final Z-axis; Assuming a spherical model  the elliptical radius of  the stars  will be conserved and the likelihood of the data $\mathcal{L}$ (Eq. \ref{eq:lnn})  is totally independent from to the rotation angles, while in an Oblate or Prolate model $\mathcal{L}$ will be  sensitive to only two rotation angles ($\eta$ and  $\beta$ for an Oblate model, $\eta$ and $\gamma$ for a Prolate model).
\item{Off-set halo:} the  elliptical radius of each star  will be  estimated  with respect to a point  off-set  by  the value ($\te{X}_\te{off}$, $\te{Y}_\te{off}$, $\te{Z}_\te{off}$) with respect to the Galactic centre.
\end{itemize}




\subsection{The method} \label{sec:method}
\subsubsection{Density of star in the observed volume}
Given  a certain halo model (Sec. \ref{sec:hmodel}), the density of stars in infinitesimal Cartesian Galactic Volume $\te{dV}_\te{g}=\te{d}\te{X}_\te{g} \te{d}\te{Y}_\te{g} \te{d}\te{Z}_\te{g}$ is  
\begin{equation}
\rho(\te{X}_\te{g}, \te{Y}_\te{g}, \te{Z}_\te{g}| \vec{\mu})=\rho_c \tilde{\rho}(\te{X}_\te{g}, \te{Y}_\te{g}, \te{Z}_\te{g}| \vec{\mu}) =\frac{\te{d}N}{\te{dV}_\te{g}},
\label{eq:drho}
\end{equation}
where $\rho_c$ is the density amplitude, $\tilde{\rho}$ is the normalised density and
$\vec{\mu}$ is the vector containing all the  model parameters  (e.g. $\vec{\mu}=(\alpha_\te{inn}, \te{q})$ for an SPL+Oblate model, see Sec. \ref{sec:hmodel}). From  $\rho$ (Eq. \ref{eq:drho}) we can  define  the quantity
\begin{equation}
\nu(m,l,b|M,\vec{\mu})= |\te{J}| \rho_c \tilde{\rho}(\te{X}_\te{g}, \te{Y}_\te{g}, \te{Z}_\te{g}| m, \te{l}, \te{b}, M, \vec{\mu}).
\label{eq:nurho}
\end{equation}
In Eq. \ref{eq:nurho}, $\nu$ is the density of stars in a infinitesimal Volume element  $\te{d}S=\te{d}m \te{d}\Omega$, where  $\te{d}\Omega=\te{dl}\te{db} \cos \te{b}$ represents the surface area element  in the sky and  $\te{d}m$ is  an infinitesimal increment of the  observed  magnitude and $|\te{J}|$  is the determinant of the Jacobian matrix  
\begin{equation}
\te{J}=\left[\frac{\te{dV}_\te{g}}{\te{d}S}\right]=\frac{1}{\cos \te{b}} \left[\frac{\te{d}\te{X}_\te{g} \te{d}\te{Y}_\te{g} \te{d}\te{Z}_\te{g}}{ \te{d}m \te{dl}\te{db} }\right].
\label{eq:finjac}
\end{equation}
The  number density $\nu$ depends also on the  additional  parameter  $M$, namely the  absolute magnitude  needed to pass from the  observed  variables  $(m, \te{l}, \te{b})$ to  the  Cartesian  variables (see Eqs. \ref{eq:amag} and \ref{eq:fref}).
Expanding  the  Jacobian determinant  (Eq. \ref{eq:appA}  in Appendix \ref{app:jaco}) in Eq. \ref{eq:nurho} we obtain  
\begin{equation}
\nu(m,l,b|M,\vec{\mu})= \frac{\ln 10}{5} \rho_c \tilde{\rho}(\te{X}_\te{g}, \te{Y}_\te{g}, \te{Z}_\te{g}| m, \te{l}, \te{b}, M, \vec{\mu}) \te{D}^3_\odot(m,M),
\label{eq:nurho2_old}
\end{equation}
and similarly to the Eq. \ref{eq:drho} we can define
\begin{equation}
\tilde{\nu}(m,l,b|M,\vec{\mu})= \tilde{\rho}(\te{X}_\te{g}, \te{Y}_\te{g}, \te{Z}_\te{g}| m, \te{l}, \te{b}, M, \vec{\mu}) \te{D}^3_\odot(m,M)
\label{eq:nurho2}
\end{equation}
that represents the normalised density in the observables space.

\subsubsection{The rate function} \label{sec:ratef}
Following  \cite{xuehalo} and \cite{bovymethod}, we can use the density function (Eq. \ref{eq:nurho2_old} and Eq. \ref{eq:nurho2}) to define  the expected rate function  for finding  a  stars  with  ($m$, l, b) given  the absolute magnitude $M$ and the halo model with  parameters  $\vec{\mu}$
\begin{equation}
\lambda(m,\te{l},\te{b},M|\vec{\mu})= \lambda_c \tilde{\lambda}(m,\te{l},\te{b},M|\vec{\mu}),
\label{eq:denslamb_b}
\end{equation}
where  $\lambda_c=\rho_c \ln 10 / 5$ is the rate amplitude and
\begin{equation}
\tilde{\lambda}(m,\te{l},\te{b},M|\vec{\mu})=\tilde{\nu}(m,\te{l},\te{b}|M, \vec{\mu}) W(m,\te{l},\te{b}| M) \Phi(M)
\label{eq:denslamb}
\end{equation}
is the normalised rate function.
In Eq. \ref{eq:denslamb}, $\Phi(M)$ represents  the distribution of  absolute magnitude of the stars, it is normalised so that the  integral (or the summation in the discrete case)  over $M$ is equal to the unity. The  function $W$ is  the selection function that takes into account the incomplete coverage of the Galactic volume:
 it is  function of l, b and $m$ (and $M$) and returns a result in the Boolean domain  B=(0, 1).  
In particular, $W$ is always equal to 1  unless  at least one  of the following conditions  comes true:
\begin{itemize}
\item  $m<G_\te{min}$,  where $G_\te{min}=10$ (Sec. \ref{sec:selection}).
\item  $m>G_\te{max}$,  where $G_\te{max}=17.1$ (Sec. \ref{sec:selection}).
\item  $|\te{b}|<10^\circ$,  this is the  cut  operated  to select the  main sample of RRLs (Sec. \ref{sec:selection});
\item $|\theta|<20^\circ$, this is the filter used to obtain the clean sample of RRLs  used in this section (Sec. \ref{sec:csample});
\item  $\te{D}_\te{LMC}<9^\circ$, where $\te{D}_\te{LMC}$ is the projected angular distance from the centre of the Large Magellanic Cloud;
\item  $\te{D}_\te{SMC}<7^\circ$, where $\te{D}_\te{SMC}$ is the projected angular distance from the centre of the Small Magellanic Cloud;
\item  $\te{l} \in [167,189] \ \te{AND} \ \te{b} \in [16,22]$;
\item  $\te{l} \in [160,190] \ \te{AND} \ \te{b} \in [63,73]$.
\end{itemize}
The  last  four conditions  take into account the mask used  to filter  the Magellanic  Clouds 
and  regions with  spurious detections of high-variability  stars, see Sec. \ref{sec:selection} for  further details.  
We can introduce an alternative normalisation scale  
\begin{equation}
\Lambda=\lambda_c \int \tilde{\lambda} \te{d} S \te{d} M =\lambda_c  \te{V}_c
\label{eq:Lambdat}
\end{equation}
that represent the expected number of stars in the whole volume $S$ marginalised over the absolute magnitude $M$ and $\te{V}_c$ is  the normalisation integral, further details can be found in Appendix \ref{app:lnlike}. 


In this work,  we decided to set the absolute magnitude of the RRLs to a single value $M_G=0.525$ (Sec. \ref{sec:amag}), so we are assuming that  $\Phi(M)$ in  Eq.   \ref{eq:denslamb_b} and  Eq.  \ref{eq:denslamb}    is  Delta of Dirac.  As a consequence, we can marginalize  Eq. \ref{eq:denslamb_b} over  $M$ and use the definition of $\Lambda$ in Eq. \ref{eq:Lambdat} to obtain  
\begin{equation}
\begin{split}
\lambda(m,\te{l},\te{b}| M_\te{G}, \vec{\mu})&=\frac{\Lambda}{\te{V}_c} \tilde{\lambda}(m,\te{l},\te{b}| M_\te{G}, \vec{\mu}) \\ 
&=\frac{\Lambda}{\te{V}_c} \tilde{\nu}(m,\te{l},\te{b}| M_\te{G}, \vec{\mu}) W(m,\te{l},\te{b}|M_\te{G}) .
\label{eq:lamnoM}
\end{split}
\end{equation}
We  notice that the  normalised rate function in Eq. \ref{eq:lamnoM} represents the  probability density function (PDF)  to find  a  stars  at certain position ($m$,\te{l},\te{b})  given the halo  parameters  $\vec{\mu}$.




%(see Appendix \ref{sec})


\subsubsection{The Likelihood} \label{sec:lkdata}

\begin{table*}
\centering
\begin{tabular}{c||ccc|ccccc}
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Model\\ component\end{tabular}} & \multicolumn{3}{c|}{Density parameters} & \multicolumn{5}{c}{Iso-density surfaces parameters} \\ \cline{2-9} 
 & $\alpha_\te{inn}$/n & $\alpha_\te{out}$ & $\te{r}_\te{eb}$ (kpc) & p & q($\te{q}_0 / \te{q}_\infty$) & $\te{r}_\te{q}$ (kpc) & $\te{X}_\te{off} / \te{Y}_\te{off} / \te{Z}_\te{off}$ (kpc) & $\eta / \beta / \gamma$ (degree) \\ \hline
\rowcolor[HTML]{C0C0C0} \hline
SPL & U{[}0,20{]} & $\delta(0)$ & $\delta(1)$ &  &  &  &  &  \\
CPL & $\delta(0)$ & U{[}0,20{]} & U{[}0.01,10{]} &  &  &  &  &  \\
\rowcolor[HTML]{C0C0C0} 
DPL & U{[}0,20{]} & U{[}0,20{]} & U{[}$\te{r}^{\te{min}}_\te{e}$,$\te{r}^{\te{max}}_\te{e}${]} $\dagger$  &  &  &  &  &  \\
BPL & U{[}0,20{]} & U{[}0,20{]} & U{[}$\te{r}^{\te{min}}_\te{e}$,$\te{r}^{\te{max}}_\te{e}${]} $\dagger$ &  &  &  &  &  \\
\rowcolor[HTML]{C0C0C0} 
Einasto & U{[}0,100{]} &  & U{[}0.1,500{]} &  &  &  &  &  \\
Spherical &  &  &  & $\delta(1)$ & $\delta(1)$ &  &  &  \\
\rowcolor[HTML]{C0C0C0} 
Oblate &  &  &  & $\delta(1)$ & U{[}0.1,10{]} &  &  &  \\
Prolate &  &  &  & U{[}0.1,10{]} & $\delta(1)$ &  &  &  \\
\rowcolor[HTML]{C0C0C0} 
Triaxial &  &  &  & U{[}0.1,10{]} & U{[}0.1,10{]} &  &  &  \\
q-var &  &  &  &  &  & U{[}0.1,100{]} &  &  \\
\rowcolor[HTML]{C0C0C0} 
Off-set &  &  &  &  &  &  & U{[}0,10{]} &  \\
Tilted &  &  &  &  &  &  &  & U{[}-80,80{]} \\ \hline
\end{tabular}
\caption{Summary of the prior distribution of the halo model parameters. Each row  is related to a given halo model component  (e.g. a density model), each column indicates a  single  parameter  or a group of parameters if they  share  the same  prior distribution.  
The U indicates  an uniform  distribution within the value shown inside the square brackets; a $\delta$ indicates a Dirac distribution, this means that the parameter  is used in the model but it is not fitted. Empty space indicates that  the parameter is not included in the model component.  
$\dagger$ The  prior range of the parameter $\te{r}_\te{eb}$  for the BPL and DPL density models  is not fixed  and it depends  on $\te{r}^{\te{min}}_\te{e}$ and  $\te{r}^{\te{max}}_\te{e}$ that  represent  the  minimum  and maximum elliptical  radius (Eq. \ref{eq:ellrad}) between the stars in our sample at given  q and p (see Sec. \ref{sec:mcmc}).
More details on the single halo model components and on the parameters can be found in Sec. \ref{sec:hmodel}.  }
\label{tab:prior}
\end{table*}

Consider  a sample of stars  $D$  with  coordinate  ($m$, l, b) and an halo model with parameters  $\vec{\mu}$. Given the PDF  $\tilde{\lambda}(\te{m}, \te{l}, \te{b})$ (Eq. \ref{eq:lamnoM})  the logarithmic likelihood  of the data given the model is
\begin{equation}
\ln\mathcal{L}(D|\vec{\mu})=   \sum^{N_\text{s}}_i \ln \frac{\tilde{\lambda}(m_i, \te{l}_i, \te{b}_i|M_\te{G}, \vec{\mu})}{\te{V}_c},
\label{eq:lnn}
\end{equation}
the detailed derivation of the logarithmic likelihood in Eq. \ref{eq:lnn} can be found in  Appendix \ref{app:lnlike}.

Using Eq.  \ref{eq:nurho2} and   Eq.  \ref{eq:lamnoM} in Eq. \ref{eq:lnn}   we obtain  the final  logarithmic likelihood
\begin{equation}
\ln\mathcal{L}(D|\vec{\mu})=   \sum^{N_\text{s}}_i \ln \frac{\tilde{\rho}_i(\te{X}_\te{g}, \te{Y}_\te{g}, \te{Z}_\te{g}| m_i, \te{l}_i, \te{b}_i, M_\te{G}, \vec{\mu}) \te{D}^3_\odot(m_i,M_\te{G})}{\te{V}_c}  
\label{eq:lnn2}
\end{equation}
where, taking into account the marginalisation over  $M$, the  normalisation integral (Eq. \ref{eq:Lambdat}) is
\begin{equation}
\te{V}_c=\int^{90^\circ}_{-90^\circ} \cos \te{b} \ \text{db}   \int^{360^\circ}_{0^\circ}   \text{dl} \int^{G_\te{max}}_{G_\te{min}} \tilde{\rho} \text{D}^3_\odot W \text{d}m.
\label{eq:vc2}
\end{equation}
Given the  property of  $W$ (Sec. \ref{sec:ratef}) the  integration in $m$ is performed  between the  magnitude range covered  by our  sample, so $G_\te{min}=10$ and  $G_\te{max}=17.1$ (see Sec. \ref{sec:selection}), while the  l-b integration is performed  through the entire sky.

The presence of the selection function $W$  complicates the estimate of  $\te{V}_c$, in fact in some regions of the integrated space,  the integrand function is not continuous and shows  abrupt decreases to 0. For this reason, the classical multi-dimensional quadrature methods are not able  to  give robust results, so  we decided  to make use  of a Monte Carlo integration technique. In particular we  used  the  \textit{vegas} algorithm \citep{vegas} through its \texttt{Python} implementation\footnote{\url{https://github.com/gplepage/vegas}}.  The final estimate of the integral  comes from  the average  of $N_\te{it}$  \textit{vegas} runs  with a $N_\te{eval}$ integrand evaluations,
The  value of  $N_\te{it}$ and $N_\te{max}$ have been chosen after  comparing the results of \textit{vegas} and  an adaptive quadrature technique\footnote{\url{https://github.com/saullocastro/cubature}} setting  $W$=1 in the integrand (Eq. \ref{eq:vc2}) looking for the best compromise between  high-precision estimate of  $\te{V}_c$ and  computational time. In particular  
we used two  settings:
\begin{itemize}
\item{$fast$} with   $N_\te{max}=10^5$ and  $N_\te{it}=20$;
\item{$robust$} with   $N_\te{max}=5\cdot10^5$ and  $N_\te{it}=100$.
\end{itemize}
See Sec. \ref{sec:mcmc} for the detailed description of how these two settings  have been used in the sampling  of  posterior probability of the halo parameters.

\subsubsection{Sampling of the parameters space} \label{sec:mcmc}
The logarithmic posterior probability  of  the  parameters $\vec{\mu}_\zeta$ of an halo  models $\zeta$ given the data is (up to a normalisation constant)
\begin{equation}
\ln\left(P\left(\vec{\mu_\zeta}|D\right)\right)= \ln\left(\mathcal{L}\left(D|\vec{\mu_\zeta}\right)\right) + \ln\left(P\left(\vec{\mu_\zeta}\right)\right),
\label{eq:likel}
\end{equation}
where  the first term in the right-hand side is the probability of the data, $D$, given the parameters $\vec{\mu}_\zeta$ and model $\zeta$ (See sec. \ref{sec:lkdata}) and the second term  represents the prior probability  of $\vec{\mu}_\zeta$ (Tab. \ref{tab:prior}). 
Using Eq. \ref{eq:lnn2} we can  write the  posterior  probability as
\begin{equation}
\begin{split}
\ln\left(P\left(\vec{\mu}_\zeta|D\right)\right) =& \sum^{N_\text{s}}_i \ln \frac{\tilde{\rho}_i(\te{X}_\te{g}, \te{Y}_\te{g}, \te{Z}_\te{g}|m_i, \te{l}_i, \te{b}_i, M_\te{G}, \vec{\mu}_\zeta) \te{D}^3_\odot(m_i,M_\te{G})}{\te{V}_c}\\   
&+ \ln\left(P\left(\vec{\mu}_\zeta\right)\right),
\end{split}
\label{eq:likel3}
\end{equation}
where  the  normalisation integral $\te{V}_c$ is defined in Eq. \ref{eq:vc2}.
We assume the prior uniform  over a quite wide range  for all the  halo parameters, details for the prior of each parameters of a given  model are specified  in  Tab. \ref{tab:prior}.  Concerning the parameter  $\te{r}_\te{eb}$ we assume, for both the BPL and DPL density models, the prior distribution  uniform between the value   $\te{r}^{\te{min}}_\te{e}$ and  $\te{r}^{\te{max}}_\te{e}$ that  represent  the  minimum  and maximum elliptical  radius (Eq. \ref{eq:ellrad}) between the stars in our sample, hence the prior range of $\te{r}_\te{eb}$  depends  on the parameters  q and  p.  Given that  for   almost all your models  q and p are approximately constrained  between  0.55 and  0.7  and  1.0 and 1.2  respectively (see Sec. \ref{sec:results}),    $\te{r}^{\te{min}}_\te{e}$ remains almost constant at 2.4 kpc, while  
$\te{r}^{\te{max}}_\te{e}$ ranges approximately  between  31 kpc and 38 kpc.


We analysed the posterior probability of the parameters $\vec{\mu}_\zeta$, for a given halo model,  using the  Eq. \ref{eq:likel3}  and sampling the parameters  space with  Goodman \& Weare's Affine Invariant Markov chain Monte Carlo (MCMC, \citealt{mcmc}) making use of the \texttt{Python}   module  emcee\footnote{\url{https://github.com/dfm/emcee}} \citep{emcee}.
The evaluation   of Eq. \ref{eq:likel3}  is  computationally expensive and the bottleneck of the process  is the  calculation of the  normalisation integral  in Eq. \ref{eq:vc2}, therefore in order to have  the best compromise between computational time and  good sampling of the parameters space we  adopted a two-stage procedure.
\begin{enumerate}
\item  In the first \vir{explorative} stage  we  sample the  parameters space using  200 walkers  with  300 steps  each after  100 \vir{burning} steps and  using the $fast$ implementation of the  normalisation integral (see Sec. \ref{sec:lkdata}). The initial positions of the walkers are randomly  chosen from their  prior distributions (Tab. \ref{tab:prior}).
\item  In the second stage  we  use 48  walkers with 300 steps and 100 \vir{burning} steps using the $robust$ implementation of the  normalisation integral (See sec. \ref{sec:lkdata}). The walkers are initially placed   in  a small regions around  the parameters for which we obtained the maximum value of the likelihood  in  the first stage.
\end{enumerate}
In the case of models with  a tilted halo   we expect to have a  lot of local  maximum  and parameters degeneration, therefore  we  introduced  also a preliminary step  in which we evaluated  the  logarithmic likelihood in a parameters grid looking for the globale maximum of the likelihood, see Sec. \ref{sec:tilt} for further details.

The  final best-fit values for the models parameters have been estimated using  the 50th percentile of the posterior distributions and  the  16th and 84th percentiles have been used to estimate the 1-$\sigma$ uncertainties.

                                         

\subsubsection{Tests on mock catalogues} \label{sec:mock}
In order to test our fitting method, we developed a simple \texttt{Python} script to generate mock catalogues with the same properties (e.g. number of stars, magnitude limits) of our clean sample of RRLs (Sec. \ref{sec:csample}) distributing the stars using a combination of density laws (Sec. \ref{sec:densmod}) and assumption on the properties of the iso-density ellipsoidal surfaces (Sec. \ref{sec:ellsurf}). We applied our fitting method to mock catalogues finding that we are able to recover nicely the input parameters for all the possible models combinations also including in the sample a fraction of contaminants coming from the Galactic disc (see Sec. \ref{sec:biasdisc} for further details).

Analysing the mock catalogues, we can predict what we  expect to measure using the stars in our catalogue. We found that we will able to detect a core on the density profile  (CPL density model) all the way down to 200-300 pc, while the detection of a change of slope depends on the halo flattening. If $\te{q}=1$, $\te{r}_\te{e}=\te{D}_\te{g}$ and we can detect a break on the density profile within about $\te{r}_\te{eb}=28$ kpc (Eq. 21), for more flattened models ($\te{q}=0.5/0.6$) this range extends up to about $\te{r}_\te{eb}=35$ kpc. However in these latter case most of the information for regions where $\te{r}_\te{e}>28$ kpc comes from a small number of stars at very high Galactic latitude, therefore the fit can be easily biased by the presence of substructures as the one highlighted in Sec. \ref{sec:vasy} and Fig. 9. 
In conclusion, we are confident to be able to robustly detect  significant  deviations from  a SPL within a range of elliptical radius coming from less than 1 kpc to about 30 kpc. 

Finally, we checked that our method can recover  a variation of the halo flattening as  found  in \cite{das} and \cite{xuehalo}.





\subsection{Results}  \label{sec:results}
In this section we  present the  main results obtained  applying the method described in Sec. \ref{sec:method}  to  the  RRLs in our clean sample (Sec. \ref{sec:csample}).

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}
\centering
\tabcolsep=0.11cm
\begin{tabular}{cc||lcc}
\hline
\multicolumn{2}{c||}{Model} & \multicolumn{1}{c}{} &  &    \\
Density law & Surface & \multicolumn{1}{c}{\multirow{-2}{*}{Parameters}}  & \multirow{-2}{*}{$\Delta \ln (\mathcal{L}_\te{max})$} & \multirow{-2}{*}{$\Delta \te{BIC}$} \\ \hline
\rowcolor[HTML]{C0C0C0} 
SPL & Sph & $\alpha_\te{inn}=2.61\pm0.01 \ (2.61)$ &  -839 & 1639 \\
SPL & Pro & $\alpha_\te{inn}=2.64\pm0.01 \ (2.64)$,   $\te{p}=1.52\pm0.03 \ (1.52)$  & -457 & 884 \\
\rowcolor[HTML]{C0C0C0} 
SPL & Obl & $\alpha_\te{inn}=2.71\pm0.01 \  (2.71)$, $\te{q}=0.58\pm0.01 \ (0.58)$ &  -52 & 75 \\
BPL & Obl & \begin{tabular}[c]{@{}l@{}}$\alpha_\te{inn}=2.70\pm0.01 \ (2.70)$, $\alpha_\te{out}=2.90\pm0.11 \ (2.87)$, \\ $\te{r}_\te{eb}=22.3^{+3.3}_{-2.8} \ (22.2)$ kpc,  $\te{q}=0.58\pm0.01 \ (0.58)$\end{tabular} &  -50 & 92 \\
\rowcolor[HTML]{C0C0C0} 
DPL & Obl & \begin{tabular}[c]{@{}l@{}}$\alpha_\te{inn}=2.70\pm0.03 \ (2.71)$, $\alpha_\te{out}=0.03^{+0.06}_{-0.02} \ (0.02)$,\\ $\te{r}_\te{eb}=21.1^{+5.7}_{-9.9} \  (23.1)$ kpc, $\te{q}=0.58\pm0.01 \ (0.58)$\end{tabular} & -52 & 94 \\
CPL & Obl & \begin{tabular}[c]{@{}l@{}}$\alpha_\te{out}=2.72\pm0.02 \ (2.71)$, $\te{r}_\te{eb}=0.03^{+0.03}_{-0.01} \ (0.03)$ kpc,  \\ $\te{q}=0.58\pm0.01 \ (0.58)$\end{tabular} &  -52 & 85 \\
\rowcolor[HTML]{C0C0C0} 
Einasto & Obl & \begin{tabular}[c]{@{}l@{}}$\te{n}=37.5^{+3.5}_{-4.6} \  (40)$, $\te{r}_\te{eb}=391.1^{+84.6}_{-169.8} \ (474)$ kpc, \\ $\te{q}=0.58\pm0.01 \ (0.58)$\end{tabular} & -58 & 96 \\
SPL & Obl+qvar & \begin{tabular}[c]{@{}l@{}}$\alpha_\te{inn}=2.93\pm0.05 \ (2.90)$, \\ $\te{q}=0.52\pm0.02 \ (0.52)$, $\te{q}_\infty=0.74\pm0.05 \ (0.75)$, \\ $\te{r}_\te{eq}=14.8\pm1.9 \ (16.3)$ kpc\end{tabular}  & -37 & 64 \\
\rowcolor[HTML]{C0C0C0} 
SPL & Tri & \begin{tabular}[c]{@{}l@{}}$\alpha_\te{inn}=2.71\pm0.01 \ (2.71)$, \\  $\te{p}=1.19\pm0.03 \ (1.19)$, $\te{q}=0.63\pm0.01 \ (0.63)$\end{tabular}  & -20 & 20 \\
SPL & Tri+qvar & \begin{tabular}[c]{@{}l@{}}$\alpha_\te{inn}=2.92\pm0.06 \ (2.92)$, $\te{p}=1.20\pm0.03 \ (1.20)$, \\ $\te{q}=0.56\pm0.02 \ (0.55)$, $\te{q}_\infty=0.84^{+0.09}_{-0.05} \ (0.82)$,\\  $\te{r}_\te{eq}=14.3^{+4.2}_{-2.6} \ (13.4)$ kpc\end{tabular}  & 0 & 0 \\ \hline
\end{tabular}
\caption{Summary of properties and results for a sample of fitted halo models. For each model we report the assumed density law (Sec. \ref{sec:densmod}) the assumed model for the shape of the  iso-density surfaces (Sec. \ref{sec:ellsurf}). For each fitted parameter  we report  the  median and  the uncertainties estimated as the 16th and 84th percentiles  of the posterior distribution, the values in parentheses indicate the value for which we obtain the maximum value of the likelihood $\mathcal{L}_\te{max}$ (Eq. \ref{eq:lnn2}) and the related BIC (Eq. \ref{eq:BIC}). 
The last columns indicate the logarithmic likelihood and BIC differences  between  the maximum (minimum for the BIC) value of the likelihood for each model and the maximum (minimum) value obtained between all the models.}
\label{tab:fit}
\end{table*}

\subsubsection{Model comparison} \label{sec:compare}
For a  given model the  MCMC sampling technique  (Sec. \ref{sec:mcmc}) gives the posterior  distributions of the model parameters. This approach  give  much more information  with respect  to  a  maximum likelihood  search method, in particular we have a  direct estimate  of the uncertainties   and of the possible  degeneration between parameters.

In addition to the estimate of the  parameters  for a single model  it is important to compare results  of different models to understand what of them gives the best description of the data. The  most  robust  way to  perform a model comparison  is  through  the  ratio of the  Bayesian evidences, it  is defined as the  integral of  the likelihood over all the parameters space. However,  this  approach could be very computationally  expensive. 
Under  the assumption that the parameters posterior distributions are almost Gaussian, the Bayesian evidence can be approximated by the  Bayesian information criterion  (BIC, \citealt{bic_def}) defined as
\begin{equation}
\text{BIC}=\dim(\vec{\mu}_\zeta)\ln\left(N_\text{S}\right) -  2 \ln\left(\mathcal{L}_\te{max}\right),
\label{eq:BIC}
\end{equation}
where  $N_\te{S}$ indicates  the number of object  in the sample  and $\mathcal{L}_\te{max}$ is the maximum value  of the likelihood  (Eq. \ref{eq:lnn2}).

The BIC is often used to compare different models with different dimensions of the parameters  space and the model with the lowest BIC is preferred (e.g. \citealt{xuehalo}). The BIC is similar to the maximum likelihood  criterion, but  it includes a  penalty depending on the number of free parameters, so that  a model to be preferred with respect a model with a lower  number of parameters  need to  improve  significantly the likelihood. 
The information on the best-fit parameters together with the maximum  likelihood and the BIC  for a representative sample  of halo models  can be found  in  Tab. \ref{tab:fit}. The  maximum  likelihoods (and the BIC) have been calculated  taking the maximum  of the  $14400$ likelihood estimates  obtained  with the final MCMC sampling of the likelihood (see Sec. \ref{sec:mcmc}).

Other than the BIC,  we also compared directly the  prediction  of    different models  with  the properties of the RRLs sample (see Sec. \ref{sec:best}). 


\subsubsection{RRLs density law} \label{sec:rrlsdl}

\begin{figure}
\centering
\includegraphics[width=1.0\columnwidth]{image/dens_func.pdf}
\caption{Radial profile of the density slope  ($\partial(\ln \rho)/\partial(\ln \te{r}_\te{e}$)) for different density law models: BPL (1th-row), DPL (2th-row), CPL (3th-row) and Einasto (4th-row).  The bands represent the samples from the posterior with edges representing 16th and 84th  percentiles. The  coloured lines represent the  median of  the posterior  fitting  only the  stars  above  ($\te{b}>10^\circ$, dotted line) and below  ($\te{b}<10^\circ$, solid line) the Galactic plane.
The dashed-black line shows the best-fit slope obtained for the SPL model. In al the case we have assumed an Oblate halo model (Tab. \ref{tab:fit}).}
\label{fig:densg}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=1.0\columnwidth]{image/dens_g.pdf}
\caption{Magnitude distribution of RRLs (Sec. \ref{sec:csample}). Top panel: the black points give the  fraction of stars 
in magnitude bins, while the coloured lines show the resultant distributions for halo models with  different density laws: SPL (blue), BPL (orange), DPL (green), CPL (red)  and Einasto (magenta). Errors bars on data points and model distributions indicate Poisson uncertainties.
Bottom panel: relative residual (Data-Model/Model), the color code is the same of the top panel and the black-dashed line indicate the 0\%.
In all the cases  we  assumed  an Oblate halo model,  the  best-fit parameters of the  models are  indicated in Tab. \ref{tab:fit}.}
\label{fig:densfunc}
\end{figure}





We tested different density profiles: the SPL (Eq. \ref{eq:plgeneral} with $\alpha_\te{out}=0$), the  DPL (Eq. \ref{eq:plgeneral}), the BPL (Eq. \ref{eq:bpl}), the CPL (Eq. \ref{eq:plgeneral} with $\alpha_\te{inn}=0$) and the Einasto profile (Eq. \ref{eq:einasto}). 

The comparison between the logarithmic maximum likelihoods and the BICs obtained for these different models are very similar  as shown in Tab. \ref{tab:fit}, therefore the DPL, BPL, CPL and Einasto models do not offer any improvement in the description of the RRLs distribution with respect to the simpler SPL.
In Tab. \ref{tab:fit} we report the comparison of different density profiles only  for an Oblate halo model, however we obtained the same results also  for Spherical, Prolate and Triaxial halo models. 

Other than  the BIC comparisons we  analysed also  the posterior distributions of the  parameters of the various density models.  For this purpose, Fig. \ref{fig:densfunc} shows the comparison between the (elliptical) radial profiles of the density slope for different halo models (coloured bands). The slopes have been calculated as the logarithmic (elliptical) radial derivative of the logarithmic density, therefore  the result for a SPL is just a constant (as shown by the black-dashed line in the four panels).
We found  that the final parameters are tuned such that  all the models tend to mimic  the properties of the  SPL  within the analysed  radial range. 


The best-fit broken radius for the BPL  is $\te{r}_\te{eb}\approx22$ kpc: in the inner part the  best-fit slope  is practically the same of the SPL model then it decreases to  a slightly larger slope of about 2.9.


Concerning the DPL, the posterior  probability of $\alpha_\te{out}$ is totally compatible  with  0, such that the final density profile is again a SPL with  a slope compatible with the best-fit SPL model (2th-row panel in Fig. \ref{fig:densfunc}). Similarly, the core radius  of the CPL model is really small (less than 100 pc), below the detectability  limit of cores for our data (see Sec. \ref{sec:mock}), therefore  
the final CPL  model is totally compatible  with  no-core  and the slope is   the same of  the  SPL model (3th-row panel in Fig. \ref{fig:densfunc}). 

Finally, for the Einasto profile  the  fit favours very large  values both for $\te{n}$ ($\approx38$) and for $\te{r}_\te{eb}$ ($\approx390$ kpc), so that  in the analysed radial range the variation of the slope is minimal  and the density profiles  can mimic as much as possible  a SPL. However using  the Einasto functional form, it  is not really  possible to reproduce a true  SPL (see 4th-row panel in Fig. \ref{fig:densfunc}), this is reflected by the fact that the BIC of the Einasto model is the largest between all the  tested density  law models.

The break radius  of  the BPL model  is  compatible with the one obtained in  \cite{xuehalo} after the subtraction of halo substructures, although the change of slope is  much more  significant  in their works with respect to our result (see Tab. \ref{tab:fitother}). It  could be possible  that the over-density of stars that we found at high  $\te{Z}_\te{g}$ (see Sec. \ref{sec:vasy}) conceals  the presence  of a drop    in the RRLs density  profile.
Instead to try to mask  the structure, that could be  a potential  subjective approach, we decide to  repeat the  likelihood sampling analysis  using  only the RRLs below and above the  Galactic  plane ($\te{b}<-10^\circ$). 
The  results   are shown in  Fig. \ref{fig:densg} by the   solid   ($\te{b}<10^\circ$) and dashed  
($\te{b}>10^\circ$)  coloured curve: in general the  stars above the Galactic plane  prefers a mean slope of about 2.65    while the  part below a of about  2.73.
Concerning  the change of slope  above the Galactic plane the posterior distribution of the BPL, DPL and CPL  models  are such as they mimic  the  SPL results, while  below the galactic plane both the BPL and  the  DPL  favours  a change of  slope, however  the BPL  is much more significant  going from about  2.73 in the inner part to  about  3.3 beyond $\te{r}_\te{e}\approx20$ kpc. It is evident  that  the stars  above the Galactic plane  have a more  shallow  decreases of the density  that  could be addressed to the  excess of  stars at high latitude. However,  also  in this  case the minimum BIC is obtained for the SPL model  indicating that  the  change of slope  is not  highly significant , moreover the fact  that the  DPL  and  the BPL show  a  significant behaviour could indicate  that  also the change of slope could be  done to some local artefact  (as  a  local decreases of the completeness). Fig. \ref{fig:densfunc} show also that the results obtained for the whole sample is almost the mean between the two analysed sub-samples.


These results point out that there are no significant evidence of deviation  from a SPL density laws, as  shown also in Fig. \ref{fig:densg}  where we compare the  fraction of RRLs in our sample in bins of observed magnitude  with the prediction of  different density models.
In conclusion the RRLs follows  a SPL  with  an exponent  that range between  2.6, assuming a Spherical halo modes, to  2.9  assuming an Oblate/Triaxial halo  with  radial variation of the flattening parameter  q. We did not find  strong evidence of  possible deviation from this SPL density profile. This  results is  in agreement  with the  estimate of the density profiles obtained in Sec. \ref{sec:rrldens} counting stars in ellipsoidal shells (Fig. \ref{sec:dprof}).
The power-law slopes   found in this work  are compatible  with  the one estimated  with  similar  sample  of  RRLs (e.g. $\alpha\approx2.8$ in \citealt{rrl3}  and  \citealt{Vivas})   although other studies found   shallower decreases  of the density (e.g. $\alpha\approx2.4$ in \citealt{watkins} or $\alpha\approx1$ within 16 kpc in \citealt{sesarhalonew}). Works using different halo tracers as BHB (\citealt{das} or \citealt{deasonhalo}) and  Giants  \citep{xuehalo} usually found a much stepper density  law ($\alpha\approx4-5$) and more significant evidence  of a change of slope  beyond 20-30 kpc,  however \cite{lamost} and \cite{xuehalo} stated  that the change of steepness found  in  their data could artificially appear  if the  radial evolution of the halo flattening is not taken into account  (see Sec. \ref{sec:isosurf}).



\subsubsection{Iso-density surfaces} \label{sec:isosurf}
As shown  by the  BIC ratios in Tab. \ref{tab:fit} the  Spherical and  Prolate models  give significantly  worst fits with respect to  the Oblate  and  Triaxial models.  
This result is confirmed by the comparison of the   properties of the RRLs in our sample with the one derived  for mock catalogues made using the best-fit parameters of the various models (Sec. \ref{sec:mock}).
For example,  Fig. \ref{fig:gdist} shows  the   fraction of  RRLs in our sample in different observed magnitude  bins (black points) compared with  the  expected distribution  for  different halo models  (assuming a SPL, see Tab. \ref{tab:fit}).  The Spherical  and the  Prolate models predict a too low fraction of stars  at lower $G$ and  a significant excess around $G=15$, while  the  Oblate and the Triaxial models  give  really a good match  to the data. 
The presence of a significant halo flattening along the  Z-axis  has been already claimed  in a large number of previous works  spanning different  halo volumes with different tracers  and  it appears to be a  very clear feature of the Galactic halo.  Contrarily, Triaxial models have not been  extensively studied so far, but  we can found some results in  \cite{deasonhalo}. They found  that a Triaxial model  increases the quality of the fit to their sample of BHB and BS,  however they  considered this result  mainly  due to an  overfit  to substructures as  Monoceros and a portion  of the Sagittarius  stream.   In our case  the  stars that can be related to Monoceros (Sec. \ref{sec:halodist})  have been cut away (Sec. \ref{sec:csample}), while  we did not find  evidence of the Sagittarius stream in the  volume  covered in this analysis.  Moreover,  the best-fit p  in \cite{deasonhalo} is  smaller than  1,  while  we found  $\te{p}\approx1.2$.  We conclude  that  the  Triaxial model  represents a real improvement  on the description of the  RRLs distribution.   

\begin{figure}
\centering
\includegraphics[width=1.0\columnwidth]{image/shape.pdf}
\caption{
As in Fig. \ref{fig:densg} but concerning halo models with different assumption of the ellipsoidal shape: Spherical (blue, $\te{q}=1$ and $\te{p}=1$), Oblate (orange, $\te{q}=0.59$ and $\te{p}=1$), Prolate (green, $\te{q}=1$ and $\te{q}=1.51$) and Triaxial (red, $\te{q}=0.63$ and $\te{p}=1.20$). 
In all the cases  we  assumed  a SPL for the density  profile  of the RRLs,  the  best-fit parameters of the  models are  indicated in Tab. \ref{tab:fit}. }
\label{fig:gdist}
\end{figure}


As  further refinement we tested Oblate and Triaxial models with  the  flattening parameter q that  can vary with the elliptical radius following the functional form in Eq. \ref{eq:qvar}. 
Allowing  q to vary, we obtained a better description of the  distribution  of RRLs as shown by the  decreases of the  BICs in Tab. \ref{tab:fit}.  The  variation of the flattening is  quite significant as it is shown in Fig. \ref{fig:qvar}:  the black curve shows the median  of the posterior probability while  the 1-$\sigma$ and 2-$\sigma$ uncertainties  are shown by the  dark and light   green bands, respectively.  The halo is largely flattened  ($\te{q}\approx0.55$) in the very inner part and then  it becomes more spherical reaching a flattening of about  0.75 at the border  of the Galactic  volume  analysed in this work  ($\te{r}_\te{e}\approx30$ kpc). 
These results are in agreement  with what we have seen directly  on 
distribution of stars in  the m-$\theta$ plane in Sec. \ref{sec:hflat} and  Fig. \ref{fig:mb10}.
As in  Sec. \ref{sec:rrlsdl} we repeated the fits using  only stars above  or below the Galactic plane and the final outcomes are totally compatible  with  the results we  obtained  with the whole sample.


Previous estimates  of  the  variation of  q (assuming the same functional form in Eq. \ref{eq:qvar}) can be found in 
\cite{das} and \cite{xuehalo}, however  they assume  that q depends on the spherical radius  $\te{D}_\te{g}$ rather than the elliptical radius $\te{r}_\te{e}$.
Nevertheless we can compare  our and their results  estimating the  value of  q  along the vertical direction  where $\te{X}_\te{g}=\te{Y}_\te{g}=0$, in this case  $\te{D}_\te{g}=\te{Z}_\te{g}$ (Eq. \ref{eq:fref2}) and  $\te{r}_\te{e} \te{q}(\te{r}_\te{e})=\te{Z}_\te{g}$ (Eq. \ref{eq:ellrad}). Therefore  at each  elliptical radius  the flattening expected from \cite{das} or \cite{xuehalo} is $\te{q}=\te{q}_\te{o}(\te{r}_\te{e} \te{q}_\te{t}(\te{r}_\te{e}))$, where $\te{q}_\te{o}$ indicate the functional forms for q that depends on $\te{D}_\te{g}$  $\te{q}_\te{t}$  is our best-fit functional forms that depends on $\te{r}_\te{e}$.
The  values of q found in this are shown  in Fig. \ref{fig:qvar} by the red \cite{das} and orange \cite{xuehalo} lines.
Both the results of  are compatible  with  our  trend of q for $\te{r}_\te{e}>15$ kpc (solid lines), but  in the  inner part (dashed lines) there is a clear discrepancy: our q is almost constant  at 0.55, while in the other works  the trend is still decreasing and the halo becomes highly flattened  ($\te{q}\approx0.4$ in \citealt{das} and $\te{q}\approx0.2$ in \citealt{xuehalo}).  Concerning these differences, we stress that  the  two  previous works have few or not stars within  10 kpc from the Galactic centre, so that our results in this region can be considered more robust.

\begin{figure}
\centering
\includegraphics[width=1.0\columnwidth]{image/qvar.pdf}
\caption{Halo flattening, q,  as function of the elliptical radius $\te{r}_\te{e}$ (Eq. \ref{eq:ellrad}). The black solid-line  shows the median of the functional-form distribution of q obtained  for the  SPL-Triaxial + q varying halo model  (last row in Tab. \ref{tab:fit})
while the related dark and light green bands indicate the 68\% and 95\% confidence intervals.  The black-dashed  line  indicates the best-fit q  obtained   for the   SPL-Triaxial+ q fix  halo model (8th row in Tab. \ref{tab:fit}). As comparison, the red and orange lines show the best-fit functional form of q found in \protect\cite{das} and  \protect\cite{xuehalo}, respectively. 
In  these works the  flattening q  is  a function of the spherical radius $\te{D}_\te{g}$ rather than the elliptical radius,  therefore to compare  their and  our results we  calculated the value of  q  along the vertical direction  where $\te{X}_\te{g}=\te{Y}_\te{g}=0$.  In this case  $\te{D}_\te{g}=\te{Z}_\te{g}$ (Eq. \ref{eq:fref2}) and  $\te{r}_\te{e} \te{q}(\te{r}_\te{e})=\te{Z}_\te{g}$ (Eq. \ref{eq:ellrad}), therefore  at each  elliptical radius  the orange and red curves  are calculated as $\te{q}=\te{q}_\te{o}(\te{r}_\te{e} \te{q}_\te{t}(\te{r}_\te{e}))$, where $\te{q}_\te{o}$ indicate the functional forms for q in \protect\cite{das} or \protect\cite{xuehalo} and $\te{q}_\te{t}$  is our results shown by the black-solid line. The solid portions of these two coloured lines indicate  robust measurements of the flattening, while the dashed portion are in a Galactic region with few or no tracers in which the flattening is not constrained ($\te{D}<10$ kpc).}
\label{fig:qvar}
\end{figure}


\subsubsection{Tilt and Off-set} \label{sec:tilt}


\begin{figure*}
\centering
\includegraphics[width=0.9\textwidth]{image/angle_dist.pdf}
\caption{Posterior distributions for the angles describing the tilt of the stellar halo with respect to the Galactic disc (see Sec. \ref{sec:ellsurf}): $\eta$ (left-hand panel) indicates the (anti-clockwise) rotation around the X-axis; $\beta$ (middle panel)  indicates the (anti-clockwise) rotation around the new Y-axis; $\gamma$ (right-hand panel)  indicates the (anti-clockwise) rotation around the final Z-axis; 
The halo model is a SPL-Triaxial + Tilt.}
\label{fig:angledist}
\end{figure*}



As  last analysis, we considered halo models  that can be  tilted with respect to the Galactic plane and off-set  from the Galactic centre (see Sec. \ref{sec:ellsurf}).
We  added these  refinements  to  the  SPL-Triaxial model  considering also the radial evolution of  the  halo flattening. 

The  posterior  distributions  of the  off-set parameters ($\te{X}_\te{off}, \te{Y}_\te{off}, \te{Z}_\te{off}$) are totally compatible with  0 and  they  are extended not  more than  about 300 pc, so we can conclude that  there are no evidence of  displacement  of the  Galactic halo with respect to the Galactic centre. 

Introducing the tilt in the Triaxial models we are just assuming that  the axes of symmetry of the halo can be oriented arbitrarily in the Galactic volume.  The  final tilt of  the halo model depends on the rotation angles $\eta$, $\beta$, $\gamma$ (see Sec. \ref{sec:ellsurf}). Unfortunately, we found that the addition of these three parameters makes the final likelihood high degenerate  and full of \vir{deep} local minimum, in this case
the  MCMC analysis tends  to explore only  a  relative  small regions  around  the  starting position on the walkers. Therefore, before to start the fit we evaluated  the  likelihood  in a  3D grid  varying $\eta$, $\beta$, $\gamma$ and leaving the other parameters fixed  to the best-fit values obtained for the Triaxial models (Tab. \ref{tab:fit}).
Exploring the  results of the grid analysis, we decided to set the initial position of the walkers in a  small regions around $\eta=\beta=\gamma=0^\circ.$

The angles for which the likelihood reaches the maximum are ($\eta$, $\beta$, $\gamma$)=(3$^\circ$, 6$^\circ$, -16$^\circ$)  and  based on the BIC analysis the tilted model indicate a substantial  improvement with respect to  the  non-tilted Triaxial model.

However, as shown in Fig. \ref{fig:angledist}, the posterior distributions of the three angles are not perfectly Gaussian: they show an extended tail toward low angles  and are all compatible with 0$^\circ$, moreover  $\gamma$   shows a very broad  posterior distribution  extended between  0$^\circ$ and 25$^\circ$ (right-hand panel in Fig. \ref{fig:angledist}).  As warned in Sec.  \ref{sec:compare} in these circumstance  the  BIC  comparison should be  used carefully. Therefore we used  mock catalogues  to compare the properties  of both  tilted and non-tilted Triaxial models. We found that the final models are very similar and  they are all capable to give a good  fit to the halo proprieties. For example,  Fig.  \ref{fig:gdist2} shows the comparison between data and different models for the magnitude distribution of the stars, the models are  a non-tilted Triaxial halo with a varying  flattening (blue curve), at  tilted Triaxial halo  with fixed q (green) and a  tilted Triaxial halo  with varyng q (red) and all of them  are capable to  give a perfect match   to the data (black points).
                        
In conclusion,  even if there are some hints about the possible  tilt of the  Galactic halo, using the current data sample  is difficult to give robust results and  we  conservatively assume  that there  is  not need of  a significant tilt to describe the RRLs distribution in the inner halo.
A  more detailed study about this interesting properties  is  postponed   in future works  in which we  will extend the coverage of the Galactic volume (see Sec. \ref{sec:future}).

\begin{figure}
\centering
\includegraphics[width=1.0\columnwidth]{image/morph.pdf}
\caption{
As in Fig. \ref{fig:densg} but concerning Triaxial halo models with varying q (blue), halo tilt (green) and  a combination of the previous models (red), see Sec. \ref{sec:tilt} for further details.}
\label{fig:gdist2}
\end{figure}



































